Dual-Glance Model for Deciphering Social Relationships

Since the beginning of early civilizations, social relationships derived from each individual fundamentally form the basis of social structure in our daily life. In the computer vision literature, much progress has been made in scene understanding, such as object detection and scene parsing. Recent research focuses on the relationship between objects based on its functionality and geometrical relations. In this work, we aim to study the problem of social relationship recognition, in still images. We have proposed a dual-glance model for social relationship recognition, where the first glance fixates at the individual pair of interest and the second glance deploys attention mechanism to explore contextual cues. We have also collected a new large scale People in Social Context (PISC) dataset, which comprises of 22,670 images and 76,568 annotated samples from 9 types of social relationship. We provide benchmark results on the PISC dataset, and qualitatively demonstrate the efficacy of the proposed model.

==> table/fig_visualize_full.tex <==
\begin{figure*}[!t]
  \centering
  \begin{minipage}{2.0\columnwidth}
   	\begin{minipage}{1.0\columnwidth} \centerline{\includegraphics[width=1.0\linewidth]{result_visualize_full}} \end{minipage}
 	\end{minipage}  	  
	\vspace{-1ex}
  \caption
    {
    \small
    Example of correct and wrongly predictions on PISC dataset. Green boxes highlight the targets, and red box highlights the contextual region with highest attention.
    }
  \label{fig:visualize_correct_wrong}
\end{figure*}

==> table/fig_visualize_non-inti.tex <==
\begin{figure*}[!t]
  \centering
	\begin{subfigure}{1\textwidth}
		\centering
		\includegraphics[width=\textwidth]{not-intimate}
		\caption{\small Not Intimate}
		\label{Not Intimate}
	\end{subfigure}
  \vspace{-1.5ex}
  \caption
    {
    \small
     Correct predictions on the test set. Green box highlights the target, red box highlights the context region with highest attention.
    }
  \label{fig:visualize_correct}
\end{figure*}

==> table/tbl_confusion_1st.tex <==
\begin{table}[!t]
	\centering
	\caption
		{
		\small	
	    Confusion matrix for the first-glance model.
		}
	\label{tbl:confusion_1st}
	\vspace{-1ex}
	\small	
	\begin{tabular}{l|c|c|c|c|c|c}
	  \toprule
	    
		& \begin{sideways} \parbox{1.8cm}{\raggedright Friends} \end{sideways} 
		& \begin{sideways} \parbox{1.8cm}{\raggedright Family Members} \end{sideways} 
		& \begin{sideways} \parbox{1.8cm}{\raggedright Couple} \end{sideways} 
	    & \begin{sideways} \parbox{1.8cm}{\raggedright Professional} \end{sideways} 
		& \begin{sideways} \parbox{1.8cm}{\raggedright Commercial} \end{sideways} 
		& \begin{sideways} \parbox{1.8cm}{\raggedright No Relation} \end{sideways} 
		\\
	  \midrule
		Friends & 30.9 & 22.2 & 25.0 & 7.1 & 4.4 & 9.4 \\
		Family Members & 8.8 & 62.9 & 13.1 & 5.1 & 3.5 & 6.7 \\
		Couple & 9.9 & 9.2 & 73.7 & 2.4 & 2.3 &2.6 \\
		Professional & 8.0 & 5.6 & 6.8 & 63.5 &6.2 & 9.8 \\
		Commercial & 7.7 & 11.3 & 10.6 & 9.7 & 43.0 & 17.6\\
		No Relation & 8.5 & 10.8 & 12.2 & 10.2 & 9.6 & 48.6\\
	  \bottomrule
	\end{tabular}
	\vspace{-2ex}
\end{table}	
		
				  


==> table/tbl_confusion_2.tex <==
\begin{table}[!t]
	\centering
	\caption
		{
		\small	
	    Confusion matrix (6-relaionship) for the dual-glance model.
		}
	\label{tbl:confusion_2}
	\vspace{-1ex}
	\small	
	\begin{tabular}{l|c|c|c|c|c|c}
	  \toprule
	    
		& \begin{sideways} \parbox{1.8cm}{\raggedright Friends} \end{sideways} 
		& \begin{sideways} \parbox{1.8cm}{\raggedright Family Members} \end{sideways} 
		& \begin{sideways} \parbox{1.8cm}{\raggedright Couple} \end{sideways} 
	    & \begin{sideways} \parbox{1.8cm}{\raggedright Professional} \end{sideways} 
		& \begin{sideways} \parbox{1.8cm}{\raggedright Commercial} \end{sideways} 
		& \begin{sideways} \parbox{1.8cm}{\raggedright No Relation} \end{sideways} 
		\\
	  \midrule
		Friends & 33.3 & 22.5 & 19.2 & 8.6 & 4.1 & 12.3 \\
		Family Members & 7.8 & 66.9 & 12.8 & 3.8 & 3.5 & 5.2 \\
		Couple & 7.9 & 8.5 & 74.9 & 4.0 & 1.6 &3.0 \\
		Professional & 11.7 & 4.8 & 5.2 & 67.4 &3.8 & 7.2 \\
		Commercial & 4.3 & 10.6 & 11.4 & 6.8 & 52.6 & 14.2\\
		No Relation & 4.9 & 8.8 & 10.3 & 9.4 & 7.9 & 58.6\\
	  \bottomrule
	\end{tabular}
	\vspace{-2ex}
\end{table}	
		
				  


==> table/tbl_confusion_dual_3class.tex <==
\newcolumntype{C}{@{\extracolsep{2pt}}c@{\extracolsep{2pt}}}%
\begin{table}[!t]
	\centering
	\caption
	{
		\small	
		Confusion matrix (3-relaionship) for the proposed dual-glance model.
	}
	\vspace{-6ex}
	\label{tbl:confusion_dual_3class}
	\small	
	
			\setlength{\arrayrulewidth}{2pt}
			\arrayrulecolor{white} 
			
	\begin{tabular}{p{1.5cm} m{0.9cm} C m{0.9cm} C  m{0.9cm} C}
		%\toprule
		
		& \begin{sideways} \rotatebox{-20}{\parbox{1.5cm}{\raggedright Intimate} }\end{sideways} 
		&
		& \begin{sideways}  \rotatebox{-20}{\parbox{1.5cm}{\raggedright Not Intimate} }\end{sideways} 
		&
		& \begin{sideways}  \rotatebox{-20}{\parbox{1.5cm}{\raggedright No Relation} }\end{sideways} 
	&
		\\
		%	\hline
		%\midrule
		\rotatebox{15}{\parbox{1.8cm}{ Intimate} } &  \cellcolor[gray]{0.279}\color{white}\bfseries{72.1}& \cellcolor[gray]{1}
		& 20.5 \cellcolor[gray]{0.795}&  \cellcolor[gray]{1}
		& 7.4 \cellcolor[gray]{0.926}&  \cellcolor[gray]{1}\\
		\hline
		\rotatebox{15}{\parbox{1.8cm}{\raggedright Not Intimate} }   
		& 9.6 \cellcolor[gray]{0.904}&  \cellcolor[gray]{1}
		& \color{white}\bfseries{83.8 }\cellcolor[gray]{0.162}&  \cellcolor[gray]{1}
		& 6.5\cellcolor[gray]{0.935}&  \cellcolor[gray]{1}\\
			\hline
		\rotatebox{15}{\parbox{1.8cm}{\raggedright No Relation} }  
		& 16.4 \cellcolor[gray]{0.836} & \cellcolor[gray]{1}
		& 23.3  \cellcolor[gray]{0.767}& \cellcolor[gray]{1}
		& \color{white}\bfseries{60.3}\cellcolor[gray]{0.397}&  \cellcolor[gray]{1}\\
		%\bottomrule
	\end{tabular}
	\vspace{-2ex}
\end{table}	
			\arrayrulecolor{black} 
			



==> table/tbl_confusion_dual_6class.tex <==
\newcolumntype{C}{@{\extracolsep{2pt}}c@{\extracolsep{2pt}}}%
\begin{table}[!t]
	\centering
	\caption
		{
		\small	
	  Confusion matrix (6-relaionship) for the proposed  dual-glance model.
		}
	\vspace{-3ex}
	\label{tbl:confusion_dual_6class}
	\small		
	\setlength{\arrayrulewidth}{2pt}
	\arrayrulecolor{white} 				
	\begin{tabular*}{.98\columnwidth}{p{1.5cm} m{0.9cm} C m{0.9cm} C  m{0.9cm} C m{0.9cm} C m{0.9cm} C m{0.9cm} C}
			& \begin{sideways} \rotatebox{-20}{\parbox{1.6cm}{\raggedright Friends} }\end{sideways} 		&
			& \begin{sideways} \rotatebox{-20}{\parbox{1.6cm}{\raggedright Family} }\end{sideways} 		&
			& \begin{sideways} \rotatebox{-20}{\parbox{1.6cm}{\raggedright Couple} }\end{sideways} 		&
	    & \begin{sideways} \rotatebox{-20}{\parbox{1.6cm}{\raggedright Professional} }\end{sideways}	    & 
			& \begin{sideways} \rotatebox{-20}{\parbox{1.6cm}{\raggedright Commercial} }\end{sideways} 		& 
			& \begin{sideways} \rotatebox{-20}{\parbox{1.6cm}{\raggedright No Relation} }\end{sideways}		&		\\
		%
		\rotatebox{15}{\parbox{1.6cm}{Friends}} 		&  \cellcolor[gray]{0.66}\color{white}\bfseries{33.3}& \cellcolor[gray]{1}
																								& 22.5 \cellcolor[gray]{0.775}&  \cellcolor[gray]{1}
																								& 19.2 \cellcolor[gray]{0.808}&  \cellcolor[gray]{1}
																								& 8.6 \cellcolor[gray]{0.914}&  \cellcolor[gray]{1}
																								& 4.1 \cellcolor[gray]{0.959}&  \cellcolor[gray]{1}
																								& 12.3 \cellcolor[gray]{0.877}&  \cellcolor[gray]{1}\\ \hline
		\rotatebox{15}{\parbox{1.6cm}{Family}}  		& 7.8 \cellcolor[gray]{0.922}&  \cellcolor[gray]{1}
																								& \color{white}\bfseries{66.9 }\cellcolor[gray]{0.331}&  \cellcolor[gray]{1}
																								& 12.8 \cellcolor[gray]{0.872}& \cellcolor[gray]{1}
																								& 3.8 \cellcolor[gray]{0.962} &  \cellcolor[gray]{1}
																								& 3.5 \cellcolor[gray]{0.967}&  \cellcolor[gray]{1}
																								& 5.2 \cellcolor[gray]{0.948}&  \cellcolor[gray]{1}\\ \hline
		\rotatebox{15}{\parbox[c]{1.6cm}{Couple}}   & 7.9 \cellcolor[gray]{0.921} & \cellcolor[gray]{1}
																								& 8.5  \cellcolor[gray]{0.915}& \cellcolor[gray]{1}
																								& \color{white}\bfseries{74.9}  \cellcolor[gray]{0.251}&  \cellcolor[gray]{1}
																								& 4.0  \cellcolor[gray]{0.96}& \cellcolor[gray]{1}
																								& 1.6 \cellcolor[gray]{.984}& \cellcolor[gray]{1}
																								& 3.0 \cellcolor[gray]{.97}&  \cellcolor[gray]{1}\\ \hline
		\rotatebox{15}{\parbox{1.6cm}{Professional}}& 11.7 \cellcolor[gray]{.883}&\cellcolor[gray]{1}
																								& 4.8 \cellcolor[gray]{.952}&\cellcolor[gray]{1}
																								& 5.2 \cellcolor[gray]{.948}&\cellcolor[gray]{1}
																								& \color{white}\bfseries{67.4} \cellcolor[gray]{.326}&\cellcolor[gray]{1}
																								& 3.8 \cellcolor[gray]{.962}&\cellcolor[gray]{1}
																								& 7.2 \cellcolor[gray]{.928}&  \cellcolor[gray]{1}\\ \hline
		\rotatebox{15}{\parbox{1.6cm}{Commercial}}	& 4.3 \cellcolor[gray]{.957}&\cellcolor[gray]{1}
																								& 10.6 \cellcolor[gray]{.894}&\cellcolor[gray]{1}
																								& 11.4 \cellcolor[gray]{.886}&\cellcolor[gray]{1}
																								& 6.8 \cellcolor[gray]{.932}&\cellcolor[gray]{1}
																								& \color{white}\bfseries{52.6} \cellcolor[gray]{.474}&\cellcolor[gray]{1}
																								& 14.2\cellcolor[gray]{.858}&  \cellcolor[gray]{1}\\ \hline
		\rotatebox{15}{\parbox{1.6cm}{No Relation}} & 4.9 \cellcolor[gray]{.951}&\cellcolor[gray]{1}
																								& 8.8 \cellcolor[gray]{.912}&\cellcolor[gray]{1}
																								& 10.3 \cellcolor[gray]{.897}&\cellcolor[gray]{1}
																								& 9.4 \cellcolor[gray]{.906}&\cellcolor[gray]{1}
																								& 7.9 \cellcolor[gray]{.921}&\cellcolor[gray]{1}
																								& \color{white}\bfseries{58.6}\cellcolor[gray]{.414}&  \cellcolor[gray]{1}\\ \hline
	\end{tabular*}
\end{table}	
		
				  


==> table/tbl_control_experiment.tex <==
\begin{table*}[!t]
	\centering
	\caption
		{
		\small	
		Accuracy .
		}
	\label{tbl:control}
	\vspace{-1ex}
	\small	
	\begin{tabular}{c|c|c|c|c|c} 
	  \toprule
		 Mean Accuracy &LC-CNN  & Pair-CNN & Pair-CNN+BBox & First-Glance & Two-Glance \\
	  \midrule
		 3-class  & 60.6\%& 65.1\%& 68.3\%& 69.7\%&\bfseries{73.1\%} \\
		 6-class  & 47.6\%& 50.2\%& 51.3\%& 53.4\%&\bf{56.9}\%\\	
	  \bottomrule
	\end{tabular}
	\vspace{-2ex}
\end{table*}	

==> table/tbl_social_relationship_tree.tex <==
\begin{table}[!t]
	\centering
	\caption
		{
		\small	
		A tree representation for the social relationship between two people.
		}
	\label{tbl:social_relationship_tree}
	\vspace{-1ex}
	\small	
	\begin{tabular}{l|l|l} 
	  \toprule
	  %\midrule
		\multirow{5}{*}{Has Relation}	&   
			\multirow{3}{*}{Intimate} & Friends \\
			& &Family Members\\ 
			& & Couple\\
			\cline{2-3}
			& \multirow{2}{*}{Not Intimate} & Professional \\
			& & Commercial\\ 
		\hline No Relation & - & -\\
	  \bottomrule
	\end{tabular}
	\vspace{-2ex}
\end{table}	

